Taming Feed-forward Reconstruction Models as Latent Encoders for 3D Generative Models

Recent AI-based 3D content creation has largely evolved along two paths: feed-forward image-to-3D reconstruction approaches and 3D generative models trained with 2D or 3D supervision. In this work, we show that existing feed-forward reconstruction methods can serve as effective latent encoders for training 3D generative models, thereby bridging these two paradigms. By reusing powerful pre-trained reconstruction models, we avoid computationally expensive encoder network training and obtain rich 3D latent features for generative modeling for free. However, the latent spaces of reconstruction models are not well-suited for generative modeling due to their unstructured nature. To enable flow-based model training on these latent features, we develop post-processing pipelines, including protocols to standardize the features and spatial weighting to concentrate on important regions. We further incorporate a 2D image space perceptual rendering loss to handle the high-dimensional latent spaces. Finally, we propose a multi-stream transformer-based rectified flow architecture to achieve linear scaling and high-quality text-conditioned 3D generation. Our framework leverages the advancements of feed-forward reconstruction models to enhance the scalability of 3D generative modeling, achieving both high computational efficiency and state-of-the-art performance in text-to-3D generation.

==> img/shapenet_con/fix_backup.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{tabular}{c c c c}
    %{c p{3.8cm} p{3.8cm} p{3.8cm}}
    
        \raisebox{0.cm}{\rotatebox{90}{\Large LN3Diff \cite{lan2025ln3diff}}}  &
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ln3diff/1b1a7af332f8f154487edd538b3d83f6.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ln3diff/1d4eaafea3ae8303ce94fde2d6224f79.png}   &
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ln3diff/1aeb17f89e1bea954c6deb9ede0648df.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ln3diff/1bcec47c5dc259ea95ca4adb70946a21.png}   & 
        \includegraphics[width=0.15\textwidth,viewport={0 256 512 768},clip]{img/shapenet_con/ln3diff/1b171503b1d0a074bc0909d98a1ff2b4.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 256 512 768},clip]{img/shapenet_con/ln3diff/1d0c128592385580e2129f6359ec27e3.png}    \\

        \raisebox{0.5cm}{\rotatebox{90}{\centering \Large Ours}} &
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ours/1b1a7af332f8f154487edd538b3d83f6.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ours/1d4eaafea3ae8303ce94fde2d6224f79.png}   &
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ours/1aeb17f89e1bea954c6deb9ede0648df.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 0 512 512},clip]{img/shapenet_con/ours/1bcec47c5dc259ea95ca4adb70946a21.png}   & 
        \includegraphics[width=0.15\textwidth,viewport={0 256 512 768},clip]{img/shapenet_con/ours/1b171503b1d0a074bc0909d98a1ff2b4.png}   
        \includegraphics[width=0.15\textwidth,viewport={0 256 512 768},clip]{img/shapenet_con/ours/1d0c128592385580e2129f6359ec27e3.png}    \\ 
        

         &
         \small \shortstack{``BMW E30 \\ race car'' } \quad \quad ``a blue car '' &
         \small \shortstack{``a four legged \\ chair with cushion''} \shortstack{``A fancy dining\\ room chair with \\sculpted wooden legs''} &
         \small \shortstack{``a green airplane \\  in the air''}  \quad \quad \shortstack{``a star wars \\ fighter jet''}
        %\small ``A clear glass mason jar with a metal lid'' & 
        %\small ``A green Christmas tree with ornaments'' & 
        %\small``A classic wooden violin with strings''  
        %\small ``A white snowman with a black top hat'' \\
    
    \end{tabular}
    \caption{ShapeNet Condition Generation Comparison. LN3Diff usually show poor resut when rendered from side view or bottom view. Zoom in for the best view. \jj{These are great, but please use powerpoint or other software to reduce the empty space and make image content larger. Also, I like the star wars plane, but the camera views are not ideal because it's hard to see the overall structure.}}
    \label{fig:text_con_compare}
\end{figure*}
  

==> img/vs_ln3diff/fig.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{tabular}{c p{3.8cm} p{3.8cm} p{3.8cm} p{3.8cm}}
        \raisebox{1.cm}{\rotatebox{90}{\Large LN3Diff \cite{lan2025ln3diff}}}  &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/012_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/032_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/043_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/052_ln3diff.png}    \\
        
        
        \raisebox{1.5cm}{\rotatebox{90}{\Large Ours}}  &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/012_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/032_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/043_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/052_ours.png}    \\

         & 
        ``A clear glass mason jar with a metal lid'' & 
        ``A green Christmas tree with ornaments'' & 
        ``A classic wooden violin with strings'' & 
        ``A white snowman with a black top hat'' \\
        
        \raisebox{1.cm}{\rotatebox{90}{\Large LN3Diff \cite{lan2025ln3diff}}}  &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/056_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/109_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/110_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/141_ln3diff.png}    \\
        
        
        \raisebox{1.5cm}{\rotatebox{90}{\Large Ours}}  &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/056_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/109_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/110_ours.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/141_ours.png}    \\

         & 
        ``A shiny red apple with a small leaf'' & 
        ``A round yellow lemon with a leaf'' & 
        ``A classic red fire hydrant'' & 
        ``A small blue recycling bin'' \\
    \end{tabular}
    \caption{Text-to-Triplane comparison}
    \label{fig:text_con_compare}
\end{figure*}

==> img/vs_ln3diff/main_fig.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{tabular}{c c c c c}
         & 
        LN3Diff \cite{lan2025ln3diff} & 
        Direct3D \cite{liu2024direct} (T=0.07) & 
        Direct3D \cite{liu2024direct} (T=0.002) & 
        Ours \\
        
         \centering {\rotatebox{90}{\small \shortstack{ ``A small blue recycling bin'' } }} &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/141_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/141_di3d1.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/141_di3d2.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/141_ours.png}    \\
        
         
         \centering{\rotatebox{90}{ \small \shortstack{``A classic red  fire hydrant'' }}}&
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/110_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/110_di3d1.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/110_di3d2.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/110_ours.png}    \\
          
        {\centering \rotatebox{90}{\small \shortstack{``A white snowman \\ with a black top hat'' }}}  &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/052_ln3diff.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/052_di3d1.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 384 384},clip]{img/vs_ln3diff/052_di3d2.png}   &
        \includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/052_ours.png}    \\
        
        
        
        %\raisebox{1.5cm}{\rotatebox{90}{\Large Ours}}  &
        %\includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/045_ours.png}   &
        %\includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/141_ours.png}   &
        %\includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/110_ours.png}   &
        %\includegraphics[width=0.21\textwidth,viewport={0 0 512 512},clip]{img/vs_ln3diff/052_ours.png}    \\

    \end{tabular}
    \caption{Text-to-Triplane comparison}
    \label{fig:text_con_compare_main_old}
\end{figure*}
